Introducing "Forecast Utterance" for Conversational Data Science

Envision an intelligent agent capable of assisting users in conducting forecasting tasks through intuitive, natural conversations, without requiring in-depth knowledge of the underlying machine learning (ML) processes. A significant challenge for the agent in this endeavor is to accurately comprehend the user's prediction goals and, consequently, formulate precise ML tasks. In this paper, we take a pioneering step towards this ambitious goal by introducing a new concept called Forecast Utterance and then focus on the automatic and accurate interpretation of users' prediction goals from these utterances. Specifically, we frame the task as a slot-filling problem, where each slot corresponds to a specific aspect of the goal prediction task. We then employ two zero-shot methods for solving the slot-filling task, namely: 1) Entity Extraction (EE), and 2) Question-Answering (QA) techniques. Our experiments, conducted with three meticulously crafted data sets, validate the viability of our ambitious goal and demonstrate the effectiveness of both EE and QA techniques in interpreting Forecast Utterances.

==> figures/heuristic_mmr.tex <==
% \vspace{-2mm}
\begin{figure}[!htb]
  \centering
    \includegraphics[width=0.9\linewidth]{images/heuristic/agg_bar.jpeg}
    \vspace{-1mm}
    \caption{MRR for Aggregation Constraint prediction.}
    \label{fig:agg_bar}

  \centering
    \includegraphics[width=0.9\linewidth]{images/heuristic/attr_bar.jpeg}
    \vspace{-1mm}
    \caption{MRR for Target Attribute prediction.}
    \label{fig:attr_bar}

  \centering
    \includegraphics[width=0.9\linewidth]{images/heuristic/filter_bar.jpeg}
    \vspace{-1mm}
    \caption{MRR for Filter Attribute prediction.}
    \label{fig:filter_bar}

  \centering
    \includegraphics[width=0.9\linewidth]{images/heuristic/filter_op_bar.jpeg}
    \vspace{-1mm}
    \caption{MRR for Filtering Constraint prediction.}
    \vspace{-2mm}
    \label{fig:filter_op_bar}
\end{figure}


==> figures/odds_comp.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/qualitative/chatgpt.jpeg}
        \label{fig:chatgpt-qual}
    \end{subfigure}
    
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/qualitative/godel.jpeg}
        \label{fig:godel-qual}
    \end{subfigure}
    
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/qualitative/vids.jpeg}
        \label{fig:vids-qual}
    \end{subfigure}
    
    \caption{}
    \label{fig:mmrs}
\end{figure}




==> figures/t5_mmr.tex <==

\begin{figure}[!htb]
  \centering
    \includegraphics[width=0.9\linewidth]{images/lm/agg.jpeg}
    \vspace{-1mm}
    \caption{MRR for Aggregation Constraint prediction.}
    \label{fig:agg_bar}

  \centering
    \includegraphics[width=0.9\linewidth]{images/lm/attr.jpeg}
    \vspace{-1mm}
    \caption{MRR for Target Attribute prediction.}
    \label{fig:attr_bar}

  \centering
    \includegraphics[width=0.9\linewidth]{images/lm/filter.jpeg}
    \vspace{-1mm}
    \caption{MRR for Filter Attribute prediction.}
    \label{fig:filter_bar}

  \centering
    \includegraphics[width=0.9\linewidth]{images/lm/filter_op.jpeg}
    \vspace{-1mm}
    \caption{MRR for Filtering Constraint prediction.}
    \vspace{-2mm}
    \label{fig:filter_op_bar}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/autoML_table.tex <==

{\clearpage
\onecolumn

\newlength{\tabfivecol}
\setlength{\tabfivecol}{\linewidth - \tabcolsep * 10}

\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\begin{longtable}{@{} @{\extracolsep{\fill}} >{\raggedright\arraybackslash}p{0.15\tabfivecol} >{\raggedright\arraybackslash}p{0.21\tabfivecol} >{\raggedright\arraybackslash}p{0.21\tabfivecol} >{\raggedright\arraybackslash}p{0.23\tabfivecol} >{\raggedright\arraybackslash}p{0.21\tabfivecol} @{}}
\caption{\label{tab:automl} A summary of contributions in the broader field of automated machine learning (AutoML). For each subtask, we list related and notable research contributions, survey articles, open source systems and commercial systems. For more details, refer to the Appendix.}\\
\toprule
Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\
\midrule
\endfirsthead
\multicolumn{5}{c}{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\
\toprule
Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\
\midrule
\endhead
\bottomrule
\endfoot
%Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\
Data Visualization,  & \citet{miao2018assessment} & \citet{ilyas2015trends} & Open Refine \uref{OpenRefine}  & Trifacta Wrangler \uref{TrifactaWrangler}\\
Cleaning and Curation & \citet{zhang2017time} & \citet{chu2016data} & Drake \uref{Drake} & TIBCO Clarity \uref{TIBCOClarity}\\
 & \citet{minnich2016clearview} &  & Open Source Data Quality and Profiling \uref{DataQuality} & Winpure \uref{Winpure}\\
 & \citet{cheng2018data} &  & Talented Data Quality  \uref{TalentedDataQuality} & Data Ladder \uref{DataLadder}\\
 & \citet{krishnan2016activeclean} &  &  & Data Cleaner \uref{DataCleaner}\\
 & \citet{chu2015katara} &  &  & Cloudingo \uref{Cloudingo}\\
 & \citet{haas2015wisteria} &  &  & Refier \uref{Refier}\\
 &  &  &  & IBM Infosphere Quality Stage \uref{IBMInfosphereQualityStage}\\
\midrule
%Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\

Feature & \citet{katz2016explorekit} & \citet{wang2005survey} & FeatureTools \uref{FeatureTools} & FeatureTools \uref{FeatureTools}\\
Engineering & \citet{kanter2015deep} & \citet{chandrashekar2014survey} & featexp \uref{featexp} & \\
 & \citet{mountantonakis2017linked} & \citet{ji2011survey} & MLFeatureSelection \uref{MLFeatureSelection} & \\
 & \citet{van2017automatic} & \citet{sheikhpour2017survey} & Feature Engineering \& Feature Selection \uref{FeatureEngineeringFeatureSelection} & \\
 & \citet{khurana2017feature} & \citet{liu2015feature} & FeatureHub \uref{FeatureHub} & \\
 & \citet{kaul2017autolearn} &  & featuretoolsR \uref{featuretoolsR} & \\
 &  &  & Feast \uref{Feast} & \\
 &  &  & ExploreKit \uref{ExploreKit} & \\
\midrule
%Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\
Hyper\-parameter  & \citet{bergstra2012random} & \citet{vanschoren2018meta} & Hyperparameter Hunter \uref{HyperparameterHunter} & Amazon Sagemaker \uref{AmazonSagemaker}\\
Tuning & \citet{snoek2012practical} & \citet{hutter2015beyond} & hyperband \uref{hyperband} & BigML OptiML \uref{BigMLOptiML}\\
 & \citet{hutter2011sequential} &  & Hyperboard \uref{Hyperboard} & Google HyperTune \uref{GoogleHyperTune}\\
 & \citet{bergstra2011algorithms} &  & SHERPA \uref{SHERPA} & Indie Solver \uref{IndieSolver}\\
 & \citet{bengio2012practical} &  & Milano \uref{Milano} & Mind Foundry OPTaaS \uref{MindFoundryOPTaaS}\\
 & \citet{bergstra2013making} &  & BBopt \uref{BBopt} & sigopt \uref{sigopt}\\
 & \citet{swersky2013multi} &  & adatune \uref{adatune} & \\
 & \citet{maclaurin2015gradient} &  & gentun \uref{gentun} & \\
 &  &  & optuna \uref{optuna} & \\
 &  &  & test-tube \uref{test-tube} & \\
 &  &  & Advisor \uref{Advisor} & \\
\midrule
%Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\

%Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\
Alternative Models  & \citet{thornton2013auto} & \citet{he2019automl} & AutoKeras \uref{AutoKeras} & H2O Driverless AI \uref{H2ODriverlessAI}\\
Exploration & \citet{feurer2015efficient} & \citet{elsken2018neural} & AdaNet \uref{AdaNet} & Cloud AutoML \uref{CloudAutoML}\\
 & \citet{swearingen2017atm} & \citet{zoller2019survey} & PocketFlow \uref{PocketFlow} & C3 AI Suite \uref{C3AISuite}\\
 & \citet{lippmann2016d3m} &  & automl-gs \uref{automl-gs} & FireFly \uref{FireFly}\\
 & \citet{zoph2016neural} &  & MLBox \uref{MLBox} & Builton \uref{Builton}\\
 & \citet{zoph2017learning} &  & Morph-net \uref{Morph-net} & Determined AI Platform \uref{DeterminedAIPlatform}\\
 & \citet{liu2017hierarchical} &  & ATM \uref{ATM} & \\
 & \citet{liu2017progressive} &  & TransmogrifAI \uref{TransmogrifAI} & \\
 & \citet{real2018regularized} &  & RemixAutoML \uref{RemixAutoML} & \\
 & \citet{pham2018efficient} &  &  & \\
 & \citet{baker2017accelerating} &  &  & \\
\midrule
%Task & Research Contributions & Survey Articles & Open Source Systems & Commercial Systems\\
Evaluation and  & \citet{shi2016benchmarking} & \citet{gijsbers2019open} & OpenML100 \uref{OpenML100} & \\
Benchmarking & \citet{Laura:2018} & \citet{klein2019meta} & OpenML-CC18 \uref{OpenML-CC18} & \\
 & \citet{duan2016benchmarking} &  & AutoML Challenges \uref{AutoMLChallenges} & \\
 & \citet{olson2017pmlb} &  &  & \\
 & \citet{eggensperger2015efficient} &  &  & \\
 
 \midrule
 Systems & \citet{swearingen2017atm} &  & Scikit-learn & DotData \uref{DotData}\\
 & \citet{golovin2017google} &  & TPOT \uref{TPOT} \cite{olson2016evaluation} & IBM AutoAI \uref{IBMAutoAI}\\
 & \citet{wang2018rafiki} &  & Auto-Sklearn \uref{Auto-Sklearn} & Azure Machine Learning \uref{AzureMachineLearning}\\
 &  &  & AlphaD3M \cite{drori2018alphad3m} & Google Could AI platform \uref{GoogleCouldAIplatform}\\
 &  &  & ML Bazaar \cite{smith2019mlbazaar} & Amazoon AWS service \uref{AmazoonAWSservice}\\
 &  &  & PyTorch & Data Robot \uref{DataRobot}\\
 &  &  &  & Amazon Forecast \uref{AmazonForecast}\\
 &  &  &  & RapidMiner \cite{hofmann2016rapidminer}\\
  &  &  &  & Orange \cite{demvsar2012orange}\\
\end{longtable}

}





==> tables/data_size.tex <==
\begin{table*}[]\small
\centering
\begin{tabular}{c|c|c|c|c|c|c}
\hline
        & \multicolumn{6}{c}{Dataset size}  \\\hline
Model   & 10592      & 21183      & 42365      & 84730      & 169460     & 338919     \\\hline
Bert    & 0.604 & 0.645 & 0.644 & 0.601 & 0.599 & 0.601 \\\hline
RoBERTa & 0.638 & 0.636 & 0.643 & 0.642 & 0.611 & 0.588 \\\hline
XLNet   & 0.664 & 0.697 & 0.666 & 0.671 & 0.669 & 0.660 \\\hline
Albert  & 0.613 & 0.617 & 0.588 & 0.614 & 0.609  & 0.585  \\\hline
Average & 0.630 & \textbf{0.649} & 0.635 & 0.632 & 0.622 & 0.608\\\hline
\end{tabular}
\caption{The F1 score of models while training on different dataset size for Entity Extraction task.}
\label{table:ee-runtime}
\end{table*}

\begin{table*}[]\small
\centering
\begin{tabular}{c|c|c|c|c|c|c}
\hline
& \multicolumn{6}{c}{Dataset size}                                          \\\hline
Model                & 10592      & 21183      & 42365      & 84730      & 169460   & 338919     \\\hline
Bert                 & 0.710 & 0.719  & 0.778 & 0.773   & 0.738    & 0.772 \\\hline
roberta              & 0.807 & 0.791 & 0.831 & 0.736 & 0.756   & 0.746 \\\hline
xlnet                & 0.598  & 0.686 & 0.644 & 0.646 & 0.622    & 0.643 \\\hline
albert               & 0.713 & 0.678 & 0.706  & 0.604  & 0.739    & 0.761 \\\hline
Average              & 0.707 & 0.718 & \textbf{0.740} & 0.690  & 0.714 & 0.731 \\\hline
\end{tabular}
\caption{The F1 score of models while training on different dataset size for Question Answering task.}
\label{table:qa-runtime}
\end{table*}

==> tables/f1_heuristic.tex <==
\begin{table*}[!htb]\small
%\begin{adjustbox}{width=\linewidth}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} &
\multicolumn{2}{c|}{\textbf{Entity Extraction}}& \multicolumn{2}{c|}{\textbf{Question Answering}} & \multicolumn{2}{c|}{\textbf{Ensemble Union}} & \multicolumn{2}{c}{\textbf{Ensemble Intersection}}\\\cline{3-10}
       &        & Universal & 	Custom  & Universal &   Custom  & Universal & Custom    & Universal & Custom  \\ \hline\hline
          
\multirow{3}{*}{\textbf{FD}}          
    & Bert      & 	0.676   & 	0.743   & \textbf{0.793}    & 	0.747       & \textbf{0.617}     & 0.657     & 0.748     & 0.738	\\\cline{2-10}
    & RoBERTa   & 	0.673   & 	0.737   & 0.753	    & 	\textbf{0.836}      & 0.595     & \textbf{0.731}     & 0.736     & \textbf{0.829}   \\\cline{2-10}
    & XLNet     & 	\textbf{0.750}   & 	0.808   & 0.619	    & 	0.666       & 0.521     & 0.615     & 0.481     & 0.343    \\\cline{2-10}
    & Albert    & 	0.657   & 	\textbf{0.817}   & 0.675	& 	0.752       & 0.491     & \textbf{0.743}     & \textbf{0.763}     & 0.782  \\\hline\hline

\multirow{3}{*}{\textbf{OD}}       
    & Bert      & 	0.625   & 	0.614   & \textbf{0.801}	& 	0.640       & \textbf{0.692}     & 0.570     & 0.730      & 0.727	\\\cline{2-10}
    & RoBERTa   & 	0.637   & 	0.619   & 0.729	    & 	\textbf{0.760}      & 0.646     & \textbf{0.706}     & \textbf{0.775}      & \textbf{0.786}   \\\cline{2-10}
    & XLNet     & 	\textbf{0.655}   & 	0.624   & 0.633	    & 	0.536       & 0.372     & 0.455     & 0.422      & 0.338    \\\cline{2-10}
    & Albert    & 	0.645   & 	\textbf{0.640}   & 0.780	& 	0.609       & 0.658     & 0.640     & 0.746      & 0.745   \\\hline\hline

\multirow{3}{*}{\textbf{SP}}   
    & Bert      & 	0.569   & 	\textbf{0.553}   & \textbf{0.610}   &   \textbf{0.639}      & 0.487      & 0.451     & 0.511     & \textbf{0.517}	\\\cline{2-10}	
    & RoBERTa   & 	0.584   & 	0.528   & 0.609	    & 	\textbf{0.628}      & \textbf{0.540}     & \textbf{0.545}      & \textbf{0.544}     & 0.490   \\\cline{2-10}
    & XLNet     & 	\textbf{0.595}   & 	0.515   & 0.582	    & 	0.472       & 0.466      & 0.456     & 0.200     & 0.338    \\\cline{2-10}
    & Albert    & 	0.564   & 	\textbf{0.541}   & 0.558	& 	0.512       & 0.451      & 0.446     & 0.500     & 0.491   \\\hline



\end{tabular}
%\end{adjustbox}
\caption{Fine-tuning performance (using \textbf{Heuristic} generated training data) on all four attributes extraction task using EE/QA and two variations of Ensemble methods.}
\label{table:ner-performence}
% \vspace{-3mm}
\end{table*}

==> tables/online_resources.tex <==


\section*{Online Resources}


\begin{urlist}
\item\label{OpenRefine}\url{http://openrefine.org/}
\item\label{TrifactaWrangler}\url{https://www.trifacta.com/products/wrangler/}
\item\label{Drake}\url{https://github.com/Factual/drake}
\item\label{TIBCOClarity}\url{https://clarity.cloud.tibco.com/landing/feature-summary.html}
\item\label{DataQuality}\url{https://sourceforge.net/projects/dataquality/})
\item\label{Winpure}\url{https://winpure.com/}
\item\label{TalentedDataQuality}\url{https://www.trustradius.com/products/talend-data-quality/reviews}
\item\label{DataLadder}\url{https://dataladder.com/}
\item\label{DataCleaner}\url{https://datacleaner.org/}
\item\label{Cloudingo}\url{https://cloudingo.com/}
\item\label{Refier}\url{http://nubetech.co/technology/}
\item\label{IBMInfosphereQualityStage}\url{https://www.ibm.com/uk-en/marketplace/infosphere-qualitystage}
\item\label{FeatureTools}\url{https://www.featuretools.com/}
\item\label{featexp}\url{https://github.com/abhayspawar/featexp}
\item\label{MLFeatureSelection}\url{https://github.com/duxuhao/Feature-Selection}
\item\label{FeatureEngineeringFeatureSelection}\url{https://github.com/Yimeng-Zhang/feature-engineering-and-feature-selection}
\item\label{FeatureHub}\url{https://github.com/HDI-Project/FeatureHub}
\item\label{featuretoolsR}\url{https://github.com/magnusfurugard/featuretoolsR}
\item\label{Feast}\url{https://cloud.google.com/blog/products/ai-machine-learning/introducing-feast-an-open-source-feature-store-for-machine-learning}
\item\label{ExploreKit}\url{https://github.com/giladkatz/ExploreKit}
\item\label{HyperparameterHunter}\url{https://github.com/HunterMcGushion/hyperparameter_hunter}
\item\label{AmazonSagemaker}\url{https://aws.amazon.com/sagemaker/}
\item\label{hyperband}\url{https://github.com/zygmuntz/hyperband}
\item\label{BigMLOptiML}\url{https://bigml.com/api/optimls}
\item\label{Hyperboard}\url{https://github.com/WarBean/hyperboard}
\item\label{GoogleHyperTune}\url{https://cloud.google.com/ml-engine/docs/using-hyperparameter-tuning}
\item\label{SHERPA}\url{https://github.com/sherpa-ai/sherpa}
\item\label{IndieSolver}\url{https://indiesolver.com/}
\item\label{Milano}\url{https://github.com/NVIDIA/Milano}
\item\label{MindFoundryOPTaaS}\url{https://www.mindfoundry.ai/mind-foundry-optimize}
\item\label{BBopt}\url{https://github.com/evhub/bbopt}
\item\label{sigopt}\url{https://sigopt.com/}
\item\label{adatune}\url{https://github.com/awslabs/adatune}
\item\label{gentun}\url{https://github.com/gmontamat/gentun}
\item\label{optuna}\url{https://github.com/optuna/optuna}
\item\label{test-tube}\url{https://github.com/williamFalcon/test-tube}
\item\label{Advisor}\url{https://github.com/tobegit3hub/advisor}
\item\label{DotData}\url{https://dotdata.com/}
\item\label{TPOT}\url{https://github.com/EpistasisLab/tpot}
\item\label{IBMAutoAI}\url{www.ibm.com/Watson-Studio/AutoAI}
\item\label{Auto-Sklearn}\url{https://github.com/automl/auto-sklearn}
\item\label{AzureMachineLearning}\url{https://azure.microsoft.com/en-us/services/machine-learning/}
\item\label{GoogleCouldAIplatform}\url{https://cloud.google.com/ai-platform/}
\item\label{AmazoonAWSservice}\url{https://aws.amazon.com/marketplace/solutions/machine-learning/data-science-tools}
\item\label{DataRobot}\url{https://www.datarobot.com/}
\item\label{AmazonForecast}\url{https://aws.amazon.com/forecast/}
\item\label{AutoKeras}\url{https://github.com/keras-team/autokeras}
\item\label{H2ODriverlessAI}\url{http://docs.h2o.ai/driverless-ai/latest-stable/docs/userguide/index.html}
\item\label{AdaNet}\url{https://github.com/tensorflow/adanet}
\item\label{CloudAutoML}\url{https://cloud.google.com/automl/}
\item\label{PocketFlow}\url{https://github.com/Tencent/PocketFlow}
\item\label{C3AISuite}\url{www.c3.ai}
\item\label{automl-gs}\url{https://github.com/minimaxir/automl-gs}
\item\label{FireFly}\url{www.firefly.ai}
\item\label{MLBox}\url{https://github.com/AxeldeRomblay/MLBox}
\item\label{Builton}\url{www.builton.dev/ml-apis}
\item\label{Morph-net}\url{https://github.com/google-research/morph-net}
\item\label{DeterminedAIPlatform}\url{www.determined.ai}
\item\label{ATM}\url{https://github.com/HDI-Project/ATM}
\item\label{TransmogrifAI}\url{https://github.com/salesforce/TransmogrifAI}
\item\label{RemixAutoML}\url{https://github.com/AdrianAntico/RemixAutoML}
\item\label{OpenML100}\url{https://www.openml.org/s/14}
\item\label{OpenML-CC18}\url{https://www.openml.org/s/98}
\item\label{AutoMLChallenges}\url{http://automl.chalearn.org/data}
\end{urlist}


